Ground Truth Inference for Weakly Supervised Entity Matching

Entity matching (EM) refers to the problem of identifying pairs of data records in one or more relational tables that refer to the same entity in the real world. Supervised machine learning (ML) models currently achieve state-of-the-art matching performance; however, they require many labeled examples, which are often expensive or infeasible to obtain. This has inspired us to approach data labeling for EM using weak supervision. In particular, we use the labeling function abstraction popularized by Snorkel, where each labeling function (LF) is a user-provided program that can generate many noisy match/non-match labels quickly and cheaply. Given a set of user-written LFs, the quality of data labeling depends on a labeling model to accurately infer the ground-truth labels. In this work, we first propose a simple but powerful labeling model for general weak supervision tasks. Then, we tailor the labeling model specifically to the task of entity matching by considering the EM-specific transitivity property. The general form of our labeling model is simple while substantially outperforming the best existing method across ten general weak supervision datasets. To tailor the labeling model for EM, we formulate an approach to ensure that the final predictions of the labeling model satisfy the transitivity property required in EM, utilizing an exact solution where possible and an ML-based approximation in remaining cases. On two single-table and nine two-table real-world EM datasets, we show that our labeling model results in a 9% higher F1 score on average than the best existing method. We also show that a deep learning EM end model (DeepMatcher) trained on labels generated from our weak supervision approach is comparable to an end model trained using tens of thousands of ground-truth labels, demonstrating that our approach can significantly reduce the labeling efforts required in EM.

==> Dependency.tex <==
\vspace{-1mm}
\section{Inferring Labeling Function Dependency} \label{lf-dep-section}



As discussed in Section~\ref{pgm-prelim-section}, the PGM requires a dependency graph $G_{dep}$ as given to specify the existence of dependency between every pair of LFs.  However, existing methods for detecting LF dependencies have multiple shortcomings as we mentioned in the introduction section. 
We overcome such shortcomings in our proposed approach by leveraging two key intuitions. 

First, two LFs may be regarded as potentially dependent only if they derive predictions based on ``overlapping information''. This is because two LFs making similar predictions using orthogonal information (e.g., from different attributes) may just be independent high-quality LFs, where treating them as dependent will unduly discount their votes. Based on this intuition, two LFs can be potentially dependent only if they access at least one shared attribute, which induces a candidate set of LF pairs that may be dependent. This intuitively leverages the input of LFs to build dependency relationships. 


Second, to figure out which pairs of LFs from the candidate set are actually dependent, we leverage an insight inspired by related work from data fusion~\cite{dongetal2009, pochampally2014}, which states that two data sources (in our analogy, LFs) are likely to be dependent if they make similar ``mistakes''. This intuitively utilizes the output of LFs to infer dependency relationships. 

When two LFs make a same mistake, the mistake is either a false positive or a false negative. 
Consider a ``positive LF'' (defined as one that only makes positive and abstain predictions) and a ``negative LF'' (which only makes negative and abstain predictions). Note that any positive LF can only make false positive mistakes, while any negative LF can only make false negative mistakes. Since a positive LF and a negative one never make the same mistake together, they should be considered as independent~\cite{dongetal2009, pochampally2014}. Following the same logic, for two LFs that make both positive and negative predictions, there can be dependency only between their positive parts, and their negative parts, respectively. 
For this reason, and to assist our reasoning of LF dependency, we conceptually ``split'' each LF into one positive LF and one negative LF, where the positive (resp. negative) part of the LF is constructed to make +1 (resp. -1) votes on the same tuple pairs as the original LF, while abstaining on all other tuple pairs.
Note that the resulting positive/negative LFs we construct from splitting LFs are no different from regular LFs that users may write manually themselves.


We are now ready to determine whether two positive/negative LFs are dependent (we only add an edge to $G_{dep}$ if so). Because it is possible that two independent LFs can make mistakes in tandem due to randomness,
we need to test whether the amount of overlap in mistakes is significantly higher than what we can expect from pure randomness. While significance is typically determined using hypothesis tests, 
there is no standard hypothesis test that applies to our scenario, so we design our own hypothesis test specifically for the LF setting. 
Designing a hypothesis test requires the following major steps~\cite{triola2014elementary}:
\begin{enumerate}[leftmargin=*]
\vspace{-2mm}
\item Identify the null hypothesis.
\item Identify the test statistic $T$.
\item Consider the proper statistical assumptions being made about the random process that generates the test statistic $T$.
\item Derive the distribution of the test statistic under the null hypothesis from the assumptions.
\item Reject the null hypothesis if the observed test statistic $\hat{T}$ is unlikely to be observed under the derived distribution, e.g. $p(T<\hat{T})<c$ where $c$ is a significance level threshold. 
\end{enumerate}

We next discuss how we proceed through each step. 

Step (1): We always prefer a sparse dependency graph to reduce the number of model parameters, so we do not consider two LFs to be dependent unless the dependency is significant. In other words, our null hypothesis is that two LFs are independent. 

Step (2): Since we want to test the significance of the dependency based on the amount of mistake overlap, our test statistic would be the amount of mistake overlap. Specifically, it is the number of data points where the two LFs both predict $+1$ (or $-1$) while the ground-truth is $-1$ (or $+1$). Obtaining this number requires the ground-truth which is not available, so we use the current inferred ground-truth. Initially, we infer the ground-truth using a PGM that assumes all LFs to be independent. After conducting the hypothesis tests and obtaining the dependency graph $G_{dep}$, the labeling model produces new inferred ground-truth labels, which are then again used to infer a new dependency graph $G_{dep}$. This process is repeated until $G_{dep}$ doesn't change. In our experiments, we observed that $G_{dep}$ converges within one or two iterations. 

Step (3) is challenging. The random process that generates the test statistic (the amount of mistake overlap) is essentially the voting process of the two LFs. The voting process depends on the internal logic of each LF and can be very complicated. Step (4) is dependent on the random process. Step (5) is straightforward. We provide the details of Step (3) in Section~\ref{ssec:voting_process} and  Steps (4)-(5) in Section~\ref{ssec:dist_mistake_overlap}.







\vspace{-3mm}
\subsection{Voting process}
\label{ssec:voting_process}










In this section, we first model the voting process of one LF, then introduce the voting process of two LFs under the null hypothesis that two LFs are independent.  Without loss of generality, we consider positive LFs (i.e., the LFs only predicts +1 and 0).

\noindent\textbf{Voting process of one LF.} 
Let $S$ denote the full set of tuple pairs. We consider a positive LF $\lambda_i$ and 
let $n_i$ denote its number of positive (+1) predictions. 
When developing the LFs, each positive LF $\lambda_i$ is written by observing a small positive subset $s_{i}$ of the tuple pairs as evidence, and the tuple pairs in the remaining set $S-s_{i}$ can be roughly divided into two groups: (1) the group that has similar patterns with $s_{i}$, where the LF $\lambda_i$ will make correct positive predictions on this group (this group contains only tuple pairs with positive ground-truth labels); and (2) the group that has different patterns from $s_{i}$ (this group can contain tuple pairs with positive and negative ground-truth labels). Since in the latter group the data differences can occur in random ways, the LF $\lambda_i$ can be considered to randomly make some positive predictions in this group.
Accordingly, the $n_i$ positive predictions of LF $\lambda_i$ can be conceptually divided into two parts: the $t_i$ positive votes on tuple pairs in group (1) that the LF is very confident about and is in fact correct, and the $r_i=n_i-t_i$ positive votes on tuple pairs in group (2) where the LF is "guessing" and can be correct or incorrect. 
In other words, we model that there is no randomness in the $t_i$ confident positive votes, while the $r_i$ positive votes can be seen to be drawn randomly among all remaining $|S|-t_i$ tuple pairs. Note that $n_i$ is observed and $t_i$ or $r_i$ is a hidden variable. Also note that $t_i$ doesn't equal the number of true positives, since making the $r_i$ random positive predictions can result in additional true positive predictions by chance. 

\noindent\textbf{Voting process of two LFs.}
To detect dependence between two positive LFs $\lambda_1$ and $\lambda_2$, we are interested in the number of overlapping incorrect predictions made by these two LFs. The overlapping incorrect predictions can only be induced by the $r_1$ and $r_2$ random positive predictions from $\lambda_1$ and $\lambda_2$, respectively. Our null hypothesis is that the two LFs are independent, i.e. the random $r_1$ positive predictions in $\lambda_1$ and the random $r_2$ positive predictions in $\lambda_2$ are made independently. Therefore, under the null hypothesis (and without loss of generality), we can have LF1 vote first and next have LF2 vote independently, i.e. the votes of LF2 are not affected by the votes made by LF1. 

Given an inferred version of the ground truth $y$ for each tuple pair in the dataset at hand.
Figure~\ref{fig:rand_pro} shows the counts of different value combinations of $\lambda_1$, $\lambda_2$ and the inferred $y$ at different stages of the voting process under the null hypothesis. $y$ has $N_{\text{pos}}$ positives and $N_{\text{neg}}$ negatives as shown in Figure~\ref{fig:rand_pro}(a). LF1 first votes its confident part of $t_1$ positive predictions with no randomness, which divides the space of $N_{\text{pos}}$ true positives into two parts (the subset where $\lambda_1$ votes and the subset where it does not), as shown in Figure~\ref{fig:rand_pro}(b). 
Note that we use red color to denote confident votes with no randomness and green color to denote the random votes of each LF. Next, in Figure~\ref{fig:rand_pro}(c), LF1 makes its $r_1$ random positive predictions which can be divided into two parts $r_{1,1}$ and $r_{1,2}$ based on the value of $y$ (+1 or -1, respectively). These votes are random in the sense that the value of $r_{1,1}$ or $r_{1,2}$ varies in different trials.
Note we use variables $z_{a,b}$ (e.g. $z_{1,2}$) to represent the complementary parts of $r_{a,b}$ variables, for example, when $r_{1,2}$ is determined, its complementary part in $N_{\text{neg}}$ is $N_{\text{neg}}-r_{1,2}$, and is represented as $z_{1,2}$. 

Once LF1 finishes, LF2 then votes its confident part of $t_2$ positives. Depending on different cases of LF1 (confident positive votes, random positive votes, and abstention), the $t_2$ votes are divided into three parts $t_{2,1}$,  $t_{2,2}$ and $t_{2,3}$ respectively, as shown in Figure~\ref{fig:rand_pro}(d). Next, LF2 makes its $r_2$ random positive votes, which are divided into five parts $r_{2,1}, \dots, r_{2,5}$ depending on the cases of LF1 and values of $y$ as shown in Figure~\ref{fig:rand_pro}(e). %
Note that Figure~\ref{fig:rand_pro}(b), Figure~\ref{fig:rand_pro}(c), Figure~\ref{fig:rand_pro}(d), and Figure~\ref{fig:rand_pro}(e) are all not observed. What can be observed is the counts for all value combinations of $\lambda_1$, $\lambda_2$, and $y$, which can be computed based on Figure~\ref{fig:rand_pro}(e) and are shown in Figure~\ref{fig:rand_pro}(f).

Note the voting process contains two types of variables $t_{a,b}$ and $r_{a,b}$ (or equivalently the complementary $z_{a,b}$ for $r_{a,b}$). The variables $r_{a,b}$ are the random variables induced by the random voting steps and they are "random variables" in the sense that they can be different with different trials of the random voting steps. In contrast, the variables $t_{a,b}$ are hidden variables that describe the intrinsic characteristics of the confident parts of two LFs, so their values are fixed though unknown. 
\begin{figure}[htb!]
  \centering
  \includegraphics[width=1\linewidth]{figures/random_process.png}
    \vspace{-7mm}
  \caption{Voting process for two LFs.}
  \label{fig:rand_pro}
     \vspace{-6mm}
\end{figure}

\vspace{-2mm}
\subsection{Distribution of mistake overlap}
\label{ssec:dist_mistake_overlap}
In this section, our goal is to derive the distribution of the amount of mistake overlap (i.e. $r_{2,4}$ in Figure~\ref{fig:rand_pro}(f)) of two LFs induced by the voting process in Section~\ref{ssec:voting_process}.
However, the voting process is still not fully determined as there are several unknown hidden variables $t_1$, $t_{2,1}$, $t_{2,2}$, and $t_{2,3}$ that describe the amount of confident votes of LF1 and LF2 (i.e. $t_1$ and $t_2 = t_{2,1}+t_{2,2}+t_{2,3}$) and how the confident votes of LF1 and LF2 intersect (i.e. $t_{2,1}$ and $t_{2,2}$). 
Our idea is to estimate these hidden variables by maximizing the likelihood of observed data, i.e. the counts in Figure~\ref{fig:rand_pro}(f).
 

\noindent\textbf{Maximum likelihood estimation of hidden variables.}
To maximize data likelihood, we need to derive the joint distribution of the observed data. We derive the joint distribution based on the two random voting steps of the two LFs. 
The first random voting step (Figure~\ref{fig:rand_pro}(b) to Figure~\ref{fig:rand_pro}(c)) induces a hyper-geometric distribution on $r_{1,1}$ and $r_{1,2}$. The second random voting step (Figure~\ref{fig:rand_pro}(d) to Figure~\ref{fig:rand_pro}(e)) induces a multi-variate hyper-geometric distribution on $r_{2,1}$, $r_{2,2}$, $r_{2,3}$, $r_{2,4}$, and $r_{2,5}$. Since we can only observe $r_{2,1} + r_{2,2}$ in Figure~\ref{fig:rand_pro}(f) (see the last two rows in the "count" column: $z_{2,1}+z_{2,2}$ and $r_{2,2}+r_{2,1}+t_{2,2}+t_{2,1}$), we rewrite the multi-variate hyper-geometric distribution to be a new multi-variate hyper-geometric distribution on $r_{2,1}+r_{2,2}$, $r_{2,3}$, $r_{2,4}$, and $r_{2,5}$. 
Under the null assumption, the two steps are independent, so multiplying the two probability distributions of the two steps gives a probability distribution of the whole voting process, which can be shown to be the joint distribution of the observed eight counts (denoted as $D$) in Figure~\ref{fig:rand_pro}(f):
\begin{small}
\begin{equation}
\label{eq:pdf}
p(D) = \frac{{N_{\text{pos}}-t_1\choose r_{1,1}}{N_{\text{neg}} \choose r_{1,2}}}{{N_{\text{pos}}+N_{\text{neg}}-t_1 \choose r_{1,1}+r_{1,2}}} 
\frac{{t_1-t_{2,1}+r_{1,1}-t_{2,2} \choose r_{2,1}+r_{2,2}}{z_{1,1}-t_{2,3}\choose r_{2,3}}{r_{1,2}\choose r_{2,4}}{z_{1,2}\choose r_{2,5}}}{{t_1-t_{2,1} + r_{1,1}-t_{2,2} +z_{1,1}-t_{2,3}+r_{1,2}+z_{1,2}\choose r_{2,1}+r_{2,2}+r_{2,3}+r_{2,4}+r_{2,5}}}
\end{equation}
\end{small}
Equation~\ref{eq:pdf} is a joint distribution on six variables : $r_{1,1}$, $r_{1,2}$, $r_{2,1}+r_{2,2}$, $r_{2,3}$, $r_{2,4}$, and $r_{2,5}$.  It can be easily shown that all the eight counts in Figure~\ref{fig:rand_pro}(f) can be represented by these six variables together with two constants ($N_{\text{neg}}$, $N_{\text{pos}}$) and four hidden variables ($t_1$, $t_{2,1}$, $t_{2,2}$, and $t_{2,3}$). 
This means that Equation~\ref{eq:pdf} is indeed the joint distribution of the observed counts in Figure~\ref{fig:rand_pro}(f).
The the values of the four hidden variables $t_1$, $t_{2,1}$, $t_{2,2}$ and $t_{2,3}$ can be estimated by maximizing the data likelihood of the observed counts i.e. $p(D)$.


\noindent\textbf{Effective size to handle voting under non-uniform randomness.} One EM-specific property is that, for a positive LF of reasonable quality, the majority of its votes should be abstention because most tuple pairs in a given EM dataset are non-matches. As a result, when choosing an LF's random positive predictions, the probability of each data point being chosen is not uniform. In particular, data points that are easy non-matches or have been blocked have nearly zero chance to be chosen. These data points are mostly the data points where $\lambda_1=0$, $\lambda_2=0$, and $y=-1$. To account for the fact that data points like these have smaller probability of being voted on, we would like to give these data points smaller weights when obtaining the counts. Let $\tilde{z_{2,5}}$ denote the count of tuple pairs where where $\lambda_1=0$, $\lambda_2=0$, and $y=-1$ \textit{after weighting}. We replace the count $z_{2,5}$ in Equation (2) with $\tilde{z_{2,5}}$ and solve $\tilde{z_{2,5}}$ by maximizing the data likelihood $p(D)$. Accordingly, $N_{\text{neg}}$ is replaced with an \textit{effective size} $\tilde{N_\text{neg}}=\tilde{z_{2,5}}+r_{2,5}+z_{2,4}+r_{2,4}$. 

\noindent\textbf{Distribution formulation for mistake overlap.} 
We have fully determined the whole voting process and can now derive the distribution of the amount of mistake overlap $p(r_{2,4})$. 
We first obtain the joint distribution $p(r_{2,4}, r_{1,2})$, as $r_{2,4}$ generated in the second random voting step is dependent on the $r_{1,2}$ that is generated in the first random voting step (see Figure~\ref{fig:rand_pro}(d) and Figure~\ref{fig:rand_pro}(e)). Again, $p(r_{2,4}, r_{1,2})$ can be obtained by multiplying two distributions induced in the two random steps:
\begin{small}
\vspace{-2mm}
\begin{equation}
\label{eq:pdf_r_24_r_12}
\begin{split}
p(r_{2,4}, r_{1,2}) =& p(r_{1,2})p(r_{2,4}|r_{1,2})\\
=& \frac{{N_{\text{pos}}-t_1 \choose r_{1,1}}{\tilde{N_\text{neg}}\choose r_{1,2}}}{{N_{\text{pos}}+\tilde{N_\text{neg}}-t_1 \choose r_{1,1}+r_{1,2}}}
\frac{{r_{1,2}\choose r_{2,4}}{N_{\text{pos}}-t_{2,1}-t_{2,2}-t_{2,3}+z_{1,2}\choose r_2-r_{2,4}}}{{N_{\text{pos}}-t_{2,1}-t_{2,2}-t_{2,3}+\tilde{N_\text{neg}}\choose r_2}} \\
=& \frac{{N_{\text{pos}}-t_1 \choose n_1-t_1-r_{1,2}}{\tilde{N_\text{neg}}\choose r_{1,2}}}{{N_{\text{pos}}+\tilde{N_\text{neg}}-t_1 \choose n_1-t_1}}
\frac{{r_{1,2}\choose r_{2,4}}{N_{\text{pos}}-t_{2,1}-t_{2,2}-t_{2,3}+\tilde{N_\text{neg}}-r_{1,2}\choose n_2-t_{2,1}-t_{2,2}-t_{2,3}-r_{2,4}}}{{N_{\text{pos}}-t_{2,1}-t_{2,2}-t_{2,3}+\tilde{N_\text{neg}}\choose n_2-t_{2,1}-t_{2,2}-t_{2,3}}}
\end{split}
\end{equation}
\end{small}
where $n_1$ and $n_2$ are the observed number of positive votes for LF1 and LF2. The only variables in Equation~\ref{eq:pdf_r_24_r_12} are $r_{2,4}$ and $r_{1,2}$, and all other values are known. Therefore, we can obtain the distribution of $r_{2,4}$ as $p(r_{2,4}) = \int p(r_{2,4}, r_{1,2}) dr_{1,2} $, and we reject the null hypothesis when the observed $\hat{r_{2,4}}$ is significantly high $
\int_{r_{2,4}>\hat{r_{2,4}}} p(r_{2,4}) dr_{2,4} < c$ where $c$ is a confidence-level threshold typically chosen as $0.05$. 
However, directly doing the integration is difficult, so we use a numerical solution. By switching the order of integration, we can obtain an equivalent form as:
\begin{equation}
\label{eq:test_lf_dependence_switch_order}
\small
\int_{r_{1,2}}\int_{r_{2,4}>\hat{r_{2,4}}} p(r_{2,4}, r_{1,2}) dr_{2,4} dr_{1,2} < c
\end{equation}
In Equation~\ref{eq:test_lf_dependence_switch_order}, for every fixed $r_{1,2}$, $p(r_{2,4},r_{1,2})$ is a hyper-geometric probability density function of $r_{2,4}$ that has a closed-form integration with respect to $r_{2,4}$. We then numerically obtain the outer integration in Equation~\ref{eq:test_lf_dependence_switch_order} by discretizing $r_{1,2}$. 


\subsection{Discussion}
The operation of inferring the hidden variables using observed data biases the random process toward the observed data in some degree, giving the null hypothesis an advantage towards not being rejected.
If the observed data still results in rejecting the null hypothesis, it is indicative of strong empirical evidence that the two LFs are not independent and we have to add an edge between the two LFs in the dependency graph. In fact, the bias toward not rejecting the null hypothesis is acceptable in our scenario as we always favor a sparse dependency structure (i.e., with fewer model parameters) unless the LFs are significantly dependent.


By applying our hypothesis test to every pair of LFs, we can construct the dependency graph $G_{dep}$ to pass to the PGM. However, recall that the M-step of PGM has a nice closed-form solution only when $G_{dep}$ is a triangulated graph; in other words, there are no minimal cycles in $G_{dep}$ of edge length greater than three. In our experiments, we observed no cases where the inferred $G_{dep}$ violated this triangularity constraint. This is because if $\lambda_1$ is detected to be dependent with $\lambda_2$ and with $\lambda_3$ by our method, it is very likely that $\lambda_2$ and $\lambda_3$ will also be detected as dependent.
However, issues could arise with this using different LFs. In this case, we can adopt a greedy approach that removes the edge between the two LFs with the least significance of mistake overlap (i.e., the value of the integration in Equation~\ref{eq:test_lf_dependence_switch_order} is the smallest) to break the large cycles.













==> Preliminaries.tex <==
\section{Preliminaries}
We review our prior interactive system (the Panda IDE)~\cite{panda_demo} for developing LFs for EM in Section \ref{dp-for-em-section}. 
Then in Section \ref{pgm-prelim-section} we formally define the problem of truth inference for EM and give an overview on the formulation of our approach. 








\subsection{An IDE for Developing LFs for EM} \label{dp-for-em-section}
Existing general-purpose data programming systems (e.g. Snorkel~\cite{2018-VLDB-Snorkel-System.pdf}) are not tailored to EM. 
To provide a specialized system for weakly supervised EM, we previously built a browser-based integrated development environment (IDE) called Panda~\cite{panda_demo} to support users as they write and debug LFs. LF development is usually an iterative trial-and-error process and is the main human cost in data programming~\cite{2016-NIPS-data-programming.pdf,2018-VLDB-Snorkel-System.pdf}.
To write LFs for EM, users need to examine tuple pairs from a specific EM task. Panda includes a smart data sampling strategy based on pre-trained language models (e.g. BERT~\cite{devlin2018bert}) to show informative tuple pairs for users to develop heuristics for writing LFs. An LF for EM typically invokes standard utility functions for pre-processing (e.g., similarity computation). Panda includes many of these commonly used utility functions to facilitate the development of LFs. Additionally, Panda automatically generates high quality LFs for users to start with by leveraging a prior unsupervised approach called Auto-FJ~\cite{AutoFJ}.

The Panda IDE integrates with the popular JupyterLab environment to support LF debugging just like in programming IDEs. Once users have written syntactically correct LFs, Panda uses a \textit{labeling model} -- the focus of this paper -- to infer ground truth labels and subsequently estimate each LF’s false positive (FP) and false negative (FN) rate. Furthermore, the IDE provides an intuitive GUI where users can point and click to quickly narrow down to the record pairs where each LF may be making mistake (i.e., disagrees with the labeling model's inferred label). Based on these record pairs, users can iteratively improve existing LFs, or choose to write new LFs that complement the existing ones.
For more details, one can refer to a demonstration video of Panda~\cite{panda_video}.



\vspace{-1mm}
\subsection{Probabilistic Modeling for Truth Inference} \label{pgm-prelim-section}
In this section, we introduce the basic formulation of our method for inferring ground truth labels, which we build on throughout the paper to account for LF dependency and tuple pair transitivity. 
 

\noindent\textbf{Problem Definition.} Given $m$ labeling functions (LFs) and $n$ tuple pairs 
to be labeled, the \textit{labeling matrix} $\Lambda \in \{+1,-1,0\}^{n \times m}$ is obtained by applying all LFs to all tuple pairs. Since LFs are noisy and may have dependencies (leading to overlaps and conﬂicts in $\Lambda$), our goal is to design and implement a \textit{labeling model} to optimally re-weight and combine the LF labels in $\Lambda$ to obtain final labeling results accurately. Formally, for each tuple pair $(t_i, t_j)$, the model should provide an estimate $\hat{y}^{(i,j)}\in\{-1, +1\}$ of the ground truth label $y^{(i,j)} \in\{-1, +1\}$. The final predictions must satisfy the transitivity constraint that if $\hat{y}^{(i,j)}$ and $\hat{y}^{(i,k)}$ are both equal to +1 (denoting matches), then $\hat{y}^{(j,k)}$ must also be +1.






\noindent\textbf{Probabilistic Graphical Model Formulation.}
Following prior work~\cite{ratner2016data}, we formulate the problem of inferring the true labels as solving a probabilistic graphical model (PGM) with a latent ground truth variable because the PGM is able to model the dependencies of the LFs in an explicit and convenient way.

Let $y$ and $\lambda = (\lambda_1, \lambda_2, \ldots, \lambda_m)$ be the random variables to denote the \textit{latent ground-truth label} and the $m$ \textit{observed labels} from $m$ LFs, respectively. 
The PGM specifies a joint probability $p_{\theta, G_{dep}}(y, \lambda)$ where $\theta$ denotes model parameters of the PGM and $G_{dep}$ is a dependency graph representing the dependencies of $(y, \lambda_1, \lambda_2, \ldots, \lambda_m)$~\cite{koller2009probabilistic}. Figure~\ref{fig:dep_graph} shows an example dependency graph. Every LF is dependent with the ground truth $y$ and is thus connected to $y$ with an edge; also, for any pair of LFs that are dependent (e.g. $\lambda_2$ and $\lambda_3$), an edge between them is added to $G_{dep}$. Deciding $G_{dep}$ is non-trivial and typical choices are either assuming no edge between any two LFs or assuming every two LFs are connected by an edge.
\begin{figure}[htb!]
  \centering
  \vspace{-3mm}
  \includegraphics[width=0.4\linewidth]{figures/dep_graph.png}
    \vspace{-3mm}
  \caption{Example dependency graph $G_{dep}$.}
  \label{fig:dep_graph}
      \vspace{-3mm}
\end{figure}

The objective function is the log data likelihood function: $L(\theta) = \sum_{(i,j)} \log p_{\theta, G_{dep}}(y^{(i,j)},\lambda^{(i,j)})$ where the superscript is used to index tuple pairs. When $y$ and $\lambda$ are both observed and $G_{dep}$ is predefined, model parameter $\theta$ is learned by maximizing the log data likelihood function $L(\theta)$. For generic dependency structure $G_{dep}$, one can use iterative optimization procedures to solve $\theta$~\cite{koller2009probabilistic}. For triangulated $G_{dep}$(i.e. for every cycle of length greater than three, there is an edge joining two nonconsecutive vertices), there exist closed form solutions under the junction tree representation~\cite{koller2009probabilistic}.

However, $G_{dep}$ is unknown and $y$ is also not observed. We must be able to automatically detect $G_{dep}$ -- failing to do so properly would result in ``double-counting" of votes from LFs that actually encode the same information, and "discounting" votes from independent LFs. Inferring the edges in $G_{dep}$ accurately presents a significant challenge and a main contribution we make (to be discussed in Section \ref{lf-dep-section}).
In our case, $y$ is not observed, so it is a latent variable and PGM with latent variables are typically learned via the expectation-maximization algorithm~\cite{koller2009probabilistic}.



\noindent\textbf{Expectation Maximization for PGM with Latent Variables.}
The Expectation Maximization algorithm executes an E-step and an M-step iteratively. 
At each E-step, the model parameter $\theta$ from the previous iteration is used to predict a soft version of $\hat{y}$, the probabilities of being a match for all tuple pairs $\boldsymbol{\gamma}$ (where each entry $\gamma^{(i,j)}= p_{\theta,G_{dep}}(y^{(i,j)}=1|\lambda^{(i,j)})$ is the posterior probability of tuple pair $(t_i, t_j)$ being a match). At each M-step, $\boldsymbol{\gamma}$ from the previous iteration is used to re-estimate $\theta$ as $\arg \max_{\theta} L(\theta)$.
The E-step is a direct invocation of inference on the PGM and can be easily done~\cite{koller2009probabilistic}. For the M-step, under generic $G_{dep}$ one has to resort iterative optimization procedure to solve $\theta$, resulting in an expensive nested iterative process (i.e. Expectation Maximization in the outer-loop and iterative optimization for $\theta$ in the inner-loop). For efficiency considerations, following prior work~\cite{fu2020fast}, we ensure $G_{dep}$ to be triangulated to enable a closed-form solution for $\theta$ under the junction-tree representation~\cite{koller2009probabilistic}. For a given dependency graph, we can easily make it triangulated by adding additional edges or removing a few edges to break large cycles~\cite{fu2020fast,koller2009probabilistic}. 






\noindent\textbf{Constrained PGM Formulation for Transitivity.}
To account for transitivity directly in the PGM, we follow prior work~\cite{ZeroER} to model transitivity as an inequality constraint defined on matching probabilities: $\gamma^{(i,j)} \times \gamma^{(i,k)} \leq \gamma^{(j,k)}$.
The set of all constraints define a \textit{feasibility set} for $\boldsymbol{\gamma}$: $Q = \{\boldsymbol{\gamma}|\gamma^{(i,j)}\gamma^{(i,k)} \leq \gamma^{(j,k)}   \forall i,j,k \}$. %

On the surface, it seems very difficult to incorporate the transitivity constraint $Q$ into the labeling model -- namely, finding the best model parameter $\theta$ that maximizes $L(\theta)$, while ensuring the probabilities $\boldsymbol{\gamma}$ computed based on $\theta$ satisfy $Q$. This conundrum is solved by using the free energy view of the expectation-maximization algorithm~\cite{neal1998view, ZeroER}. In this view, the objective function becomes the the free energy function $F(\boldsymbol{\gamma},\theta)$ that treats both $\theta$ and $\boldsymbol{\gamma}$ as its two separate sets of parameters: 
\begin{equation}
\label{eq:free_energy}
\small
\begin{split}
        F(\boldsymbol{\gamma},\theta) =& \sum_{(i,j)}  \boldsymbol{\gamma}^{(i,j)}\log\big(p_{\theta,G_{dep}}(y^{(i,j)}=1,\lambda^{(i,j)})/ \boldsymbol{\gamma}^{(i,j)}\big)\\
        +&(1-\boldsymbol{\gamma}^{(i,j)})\log\big(p_{\theta,G_{dep}}(y^{(i,j)}=-1,\lambda^{(i,j)})/ (1-\boldsymbol{\gamma}^{(i,j)})\big)\\
\end{split}
\end{equation}
The M-step stays the same as it was before, while the E-step also becomes an optimization process that allows us to incorporate the transitivity constraints. Specifically, in the E-step, we find the best $\boldsymbol{\gamma}$ that satisfies $Q$, namely $\boldsymbol{\gamma} = \arg \max_{\boldsymbol{\gamma} \in Q} F(\boldsymbol{\gamma},\theta)$.
However, $\arg \max_{\boldsymbol{\gamma} \in Q} F(\boldsymbol{\gamma},\theta)$ is difficult to solve since the constraint set $Q$ is actually non-convex (the Hessian matrix of a constraint is indefinite)~\cite{ZeroER}. Existing work uses a projection-based heuristic~\cite{ZeroER}, which is not robust across datasets as we show in experiments. We propose a more principled solution in Section~\ref{tup-trans-section}. 

